A Model for Understanding and Reducing Developer Burnout

Job burnout is a type of work-related stress associated with a state of physical or emotional exhaustion that also involves a sense of reduced accomplishment and loss of personal identity. Burnt out can affect one's physical and mental health and has become a leading industry concern and can result in high workforce turnover. Through an empirical study at Globant, a large multi-national company, we created a theoretical model to evaluate the complex interplay among organizational culture, work satisfaction, and team climate, and how they impact developer burnout. We conducted a survey of developers in software delivery teams (n=3281) to test our model and analyzed the data using structural equation modeling, moderation, and multi-group analysis. Our results show that Organizational Culture, Climate for Learning, Sense of Belonging, and Inclusiveness are positively associated with Work Satisfaction, which in turn is associated with Reduced Burnout. Our model generated through a large-scale survey can guide organizations in how to reduce workforce burnout by creating a climate for learning, inclusiveness in teams, and a generative organizational culture where new ideas are welcome, information is actively sought and bad news can be shared without fear.

==> Tables/cronbach_cr.tex <==
\begin{table}[!hb]
\centering
\caption{Internal Consistency Reliability}
\label{tab:internal_consistency_reliability}
\robustify{\bfseries}
\sisetup{
    mode=text,
    group-digits = false ,
    input-signs ={-},
    input-symbols = ( ) [ ] - + *,
    detect-weight=true, 
    detect-family=true,
    table-format=0.2,
    add-decimal-zero=false, %% doesn't seem to work :-(
    add-integer-zero=false,
    round-mode=places, 
    round-precision=2, %% change this for precision.
    parse-numbers = true
}
\begin{tabular}{L{4cm}
                S
                S
                S}
\toprule
& {\makecell{Cronbach's \textalpha}} & {\makecell{CR}} & {AVE}\\

\midrule
Organizational Culture (OC) & .82 & .87 & .77\\
%\midrule
%\addlinespace
Climate for Learning (CL) & .71 & .87 & .53\\
%\addlinespace
Work Satisfaction (SAT) & .73 & .85 & .65\\
%\addlinespace
Burnout (BNT) & .70 & .87 & .77\\
\bottomrule


%\resizebox{0.9\textwidth}{!}{%
%\begin{tabular}{|l|l|l|l|}
%\hline
%& {\cellcolor[HTML]{C0C0C0}Cronbach's Alpha} & {\cellcolor[HTML]{C0C0C0}Composite Reliability} & {\cellcolor[HTML]{C0C0C0}Average Variance Extracted (AVE)}\\ \hline
%{\cellcolor[HTML]{C0C0C0}English confidence} & 0.930 & 0.950 & 0.826               \\ \hline
%{\cellcolor[HTML]{C0C0C0}SVC}                 & 0.756 & 0.834 & 0.505              \\ \hline
%\end{tabular}}

\end{tabular}
\end{table}

==> Tables/cross_loadings.tex <==
\begin{table}[!htb]
\centering
\caption{Cross loadings of the retained indicators on the latent constructs}
\label{tab:cross_loadings}
\robustify{\bfseries}
\sisetup{
    mode=text,
    group-digits = false ,
    input-signs ={-},
    input-symbols = ( ) [ ] - + *,
    detect-weight=true, 
    detect-family=true,
    table-format=0.2,
    add-decimal-zero=false, %% doesn't seem to work :-(
    add-integer-zero=false,
    round-mode=places, 
    round-precision=2, %% change this for precision.
    parse-numbers = true
}
\begin{tabular}{p{1cm}
                p{1.4cm}
                p{1.4cm}
                p{1.4cm}
                p{1cm}}
\toprule
Item & {Organizational Culture (OC)} & {Climate for Learning (CL)} & {Work Satisfaction (SAT)} & {Burnout (BNT)}\\
\midrule
{OC1} & \textbf{.70} & .34 & .34 & .35\\
{OC2} & \textbf{.70} & .39 & .38 & .36\\
{OC3} & \textbf{.76} & .42 & .43 & .40\\
{OC4} & \textbf{.74} & .44 & .42 & .36\\
{OC5} & \textbf{.75} & .39 & .41 & .42\\
{OC6} & \textbf{.71} & .37 & .36 & .36\\
{CL1} & .51 & \textbf{.89} & .41 & .37\\
{CL2} & .44 & \textbf{.87} & .42 & .32\\
{SAT1} & .47 & .45 & \textbf{.87} & .41 \\
{SAT2} & .46 & .39 & \textbf{.82} & .45 \\
{SAT3} & .36 & .29 & \textbf{.73} & .29 \\
{BNT1} & .41 & .31 & .41 & \textbf{.86} \\
{BNT2} & .49 & .38 & .44 & \textbf{.89} \\

\bottomrule


\end{tabular}
\end{table}

==> Tables/effect_size.tex <==
\begin{table}[htb]
\centering
\caption{Effect sizes for all constructs (with specified endogenous variable to which the effect size applies)}
\label{tab:effect_size}

\sisetup{
    table-format=1.3,
    mode=text,
    detect-weight=true, 
    detect-family=true,
    add-decimal-zero=false, %% doesn't seem to work :-(
    add-integer-zero=false,
    round-mode=places, 
    round-precision=3 %% change this for precision.
}
\begin{tabular}{p{7cm}S}
\toprule
{Hypotheses} & {\textit{f}\textsuperscript{2}}\\
\midrule

(H1) Kinship, Altruism $\rightarrow$ SVC & .042\\
\addlinespace
(H2) Fun $\rightarrow$ SVC & .059\\
\addlinespace
(H3) Ideology, Reciprocity $\rightarrow$ SVC & .004\\
\addlinespace
(H4a) Power Distance X Kinship,Altruism $\rightarrow$ SVC & 0.023\\
\addlinespace
(H4b) Power Distance X Fun $\rightarrow$ SVC  & .003 \\
\addlinespace
(H4c) Power Distance X Ideology, Reciprocity $\rightarrow$ SVC & .002\\
\addlinespace
(H5a) Is paid X Kinship $\rightarrow$ SVC & .001  \\ 
\addlinespace
(H5b) Is paid X Fun $\rightarrow$ SVC & .025  \\ 
\addlinespace
(H5c) Is paid X Ideology $\rightarrow$ SVC & .001 \\ 
\midrule
\textsc{Control Variables}&\\
\midrule 
Gender Minorities $\rightarrow$ SVC    & .028 \\ 
\addlinespace
English Confidence $\rightarrow$ SVC & .026 \\ 
\addlinespace
Tenure $\rightarrow$ SVC & .081\\
\bottomrule
\end{tabular}

%\resizebox{0.7\textwidth}{!}{%
%\begin{tabular}{|ll|}
%\hline
%\multicolumn{1}{|l|}{}                                                              & {\cellcolor[HTML]{C0C0C0}\textbf{Effect Sizes}} \\ \hline
%\multicolumn{2}{|l|}{\textbf{Hypotheses}}                                                                   \\ \hline
%\multicolumn{1}{|l|}{(H1) Kinship/Altruism \rightarrow SVC} & 0.042 \\ \hline
%\multicolumn{1}{|l|}{(H2) Fun \rightarrow SVC} & 0.059 \\ \hline
%\multicolumn{1}{|l|}{(H3) Ideology/Reciprocity \rightarrow SVC} & 0.004 \\ \hline
%\multicolumn{1}{|l|}{(H4a) Power Distance X Kinship/Altruism \rightarrow SVC} & 0.023  \\ \hline
%\multicolumn{1}{|l|}{(H4b) Power Distance X Fun \rightarrow SVC} & 0.003 \\ \hline
%\multicolumn{1}{|l|}{(H4c) Power Distance X Ideology/Reciprocity \rightarrow SVC}  & 0.002 \\ \hline
%\multicolumn{1}{|l|}{(H5a) Is paid X Kinship/Altruism \rightarrow SVC} & 0.001 \\ \hline
%\multicolumn{1}{|l|}{(H5b) Is paid X Fun \rightarrow SVC}                         & 0.025 \\ \hline
%\multicolumn{1}{|l|}{(H5c) Is paid X Ideology/Reciprocity \rightarrow SVC}                    & 0.001                 \\ \hline
%\multicolumn{2}{|l|}{\textbf{Control Variables}}                                                            \\ \hline
%\multicolumn{1}{|l|}{Gender Minorities \rightarrow SVC}                           & 0.028 \\ \hline
%\multicolumn{1}{|l|}{English confidence \rightarrow SVC}                         & 0.026 \\ \hline
%\multicolumn{1}{|l|}{Tenure \rightarrow SVC}                                    & 0.081 \\ \hline
%\end{tabular}}

\end{table}

==> Tables/fornell-larcker.tex <==
\begin{table}[tbh]
\centering
\caption{Fornell-Larcker criterion: correlations among the constructs and square roots of the AVE values (on diagonal)}
\label{tab:fornell-larcker}

\begin{tabular}{p{1cm}
                p{1.4cm}
                p{1.4cm}
                p{1.4cm}
                p{1cm}}
\toprule
& {Organizational Culture (OC)} & {Climate for Learning (CL)} & {Work Satisfaction (SAT)} & {Burnout (BNT)}\\
\midrule
{OC} & \textbf{.73} &  &  & \\
%\addlinespace
{CL} &  .54 & \textbf{.88} &  &  \\
%\addlinespace
{SAT} & .54 & .47 & \textbf{.81} & \\
%\addlinespace
{BNT} & .52 &  .40 &  .48 & \textbf{.88}\\
\bottomrule



\end{tabular}
\end{table}

==> Tables/ipma.tex <==
\begin{table}[!b]
\centering
\caption{Constructs Importance and Performance referred to Burnout}
\label{tab:ipma}
\robustify{\bfseries}
\sisetup{
    mode=text,
    group-digits = true,
    group-separator={,},
    group-minimum-digits=4,
    detect-weight=true, 
    detect-family=true,
    round-mode=places, 
    round-precision=2
}
\begin{tabular}{p{3cm}
                S[table-format=1.2]
                S[table-format=2.2]}
\toprule
Construct & {Importance} & {Performance}\\
\midrule
Organizational Culture & .19 & 86.45 \\
Belonging & .15 & 81.96 \\
Climate for Learning & .15 & 88.81 \\
Inclusiveness & .10 & 92.411 \\
Work Satisfaction & .48 & 87.46 \\
%Burnout & & 78.79 \\
\midrule
Indicator & {Importance} & {Performance}\\
\midrule
OC1 & 0.043 & 88.80 \\
OC2 & 0.043 & 82.83 \\
OC3 & 0.047 & 84.84 \\
OC4 & 0.047 & 89.33 \\
OC5 & 0.044 & 85.42 \\
OC6 & 0.042 & 86.61 \\
CL1 & 0.086 & 88.01 \\
CL2 & 0.080 & 89.64 \\
SAT1 & 0.209 & 86.26 \\
SAT2 & 0.213 & 86.13 \\
SAT3 & 0.175 & 89.912 \\
\bottomrule

\end{tabular}

\end{table}

==> Tables/mga_leaders.tex <==
\begin{table}[b]
\centering
\caption{Multi-Group Analysis per Leadership Position: coefficients in bold are significant; 
lines in gray show significant difference between segments}
\label{tab:mga_leaders}
\robustify{\bfseries}
\sisetup{
    mode=text,
    group-digits = false ,
    input-signs ={-},
    input-symbols = ( ) [ ] - + *,
    detect-weight=true, 
    detect-family=true,
    table-format=0.2,
    add-decimal-zero=false, %% doesn't seem to work :-(
    add-integer-zero=false,
    round-mode=places, 
    round-precision=2, %% change this for precision.
    parse-numbers = true
}
\begin{tabular}{L{5cm}
                S[table-format=0.3]
                S[table-format=0.2]
                S[table-format=0.1]}

\toprule

& {No-Leaders} & {Leaders} & {All}\\

\midrule
Sample size (N) & {2,982} & {299} & {3,281}\\
\midrule 
%\addlinespace
Belonging (\textit{R}\textsuperscript{2}) & .23 & .24 & .23\\
%\addlinespace
\midrule 
Climate for Learning (\textit{R}\textsuperscript{2}) & \bfseries{.28} & \bfseries{.32} & \bfseries{.29}\\
%\addlinespace
\midrule 
Inclusiveness (\textit{R}\textsuperscript{2}) & \bfseries{.17} & \bfseries{.28} & \bfseries{.20}\\
%\addlinespace
\midrule 
Work Satisfaction (\textit{R}\textsuperscript{2}) & .38 & .41 & .39\\
%\addlinespace
\midrule 
Burnout (\textit{R}\textsuperscript{2}) & .31 & .37 & .33\\
%\addlinespace
\midrule 
\hangindent1em H1 Organizational Culture $\rightarrow$ Belonging & \bfseries{.47} & \bfseries{.50} & \bfseries{.48}\\ 
%\hline
%\addlinespace 
\hangindent1em H2 Organizational Culture$\rightarrow$Climate for Learning & \bfseries{.54} & \bfseries{.56} & \bfseries{.54}\\ 
%\hline
%\addlinespace 
\hangindent1em H3 Organizational Culture$\rightarrow$Inclusiveness & \bfseries{.44} & \bfseries{.46} & \bfseries{.45}\\ 
%\hline
%\addlinespace 

\hangindent1em H4 Belonging $\rightarrow$ Work Satisfaction & \bfseries{.24} & \bfseries{.20} & \bfseries{.24}\\ 
%\hline
%\addlinespace 
\rowcolor{vlightgray}\hangindent1em H5 Climate for Learning $\rightarrow$ Work Satisfaction  & \bfseries{.22} & .08 & \bfseries{.22}\\
%\hline
%\addlinespace 
\hangindent1em H6 Inclusiveness $\rightarrow$ Work Satisfaction & \bfseries{.13} & .01 & \bfseries{.12}\\ 
%\hline
%\addlinespace 
\hangindent1em H7 Work Satisfaction $\rightarrow$ Burnout & \bfseries{-.29} & \bfseries{-.20} & \bfseries{-.29}\\

\midrule
Moderators & & &\\
\midrule
\hangindent1em H8.a Power distance \texttimes{} Work Satisfaction $\rightarrow$ Burnout & .11 & .07 & .08\\
\hangindent1em H8.b Individualism \texttimes{} Work Satisfaction $\rightarrow$ Burnout & .16 & .03 & .05\\
\hangindent1em H8.c Masculinity \texttimes{} Work Satisfaction $\rightarrow$ Burnout & -.17 & .01 & -.02\\
\hangindent1em H8.d Uncertainty Avoidance \texttimes{} Work Satisfaction $\rightarrow$ Burnout & -.01 & .01 & -.01\\
\hangindent1em H8.e Long Term Orientation \texttimes{} Work Satisfaction $\rightarrow$ Burnout & -.10 & -.06 & -.09\\
\hangindent1em H8.b Indulgence \texttimes{} Work Satisfaction $\rightarrow$ Burnout & .15 & -.04 & -.02\\

\bottomrule

\end{tabular}
\vspace{-3mm}
\end{table}


==> formatting.tex <==
%%
%% Klaas's secret formatting code.
%%
\usepackage{bookmark}
\usepackage[authoryear]{natbib}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{microtype}
\usepackage{booktabs}
\usepackage[mode=text]{siunitx}
\usepackage{etoolbox}
\usepackage{enumitem} 
\usepackage{textgreek}
\usepackage{tipa}
\usepackage{url}
\usepackage{ragged2e}
\usepackage{caption}
\usepackage{times}


%\captionsetup[table]{font=footnotesize,labelfont={bf,sf},labelsep=quad,justification=RaggedRight,singlelinecheck=0}

\captionsetup[figure]{font=footnotesize,labelfont={sf,bf},labelsep=period,singlelinecheck=0,margin=0pt}



\widowpenalty10000
\clubpenalty10000

\newcolumntype{P}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}
\usepackage{makecell}

\newcommand\hypothesis[2]{\vspace{0.5em} \noindent \hangindent=1em \textbf{Hypothesis #1 (H#1).} {#2}\vspace{0.5em}}



\usepackage[
paperwidth=15.51cm,
paperheight=23.52cm,
margin=0.65in
]{geometry}


\usepackage{hyperref}
\hypersetup{
 colorlinks=true,   
 citecolor=blue,
 urlcolor=blue,
 linkcolor=blue,
 bookmarksnumbered=true,     
 bookmarksopen=true,         
 bookmarksopenlevel=1,       
 colorlinks=true,            
 pdfstartview=Fit,           
 pdfpagemode=UseOutlines,    
 pdfpagelayout=TwoPageRight 
}

\usepackage{titlesec}

\usepackage[lining]{FiraSans} 
\usepackage[T1]{fontenc}

\titleformat{\section}
  {\sffamily\bfseries\fontsize{11}{13}\selectfont}{\thesection}{1em}{}

\titleformat{\subsection}
  {\sffamily\bfseries\fontsize{10}{12}\selectfont}{\thesubsection}{1em}{}

\titleformat{\subsubsection}
  {\sffamily\bfseries\itshape\fontsize{9}{11}\selectfont}{\thesubsubsection}{0.5em}{}



==> leftOver.tex <==
ABSTRACT
%Ensuring the well-being of software developers has never been more important as the COVID-19 pandemic has forced a majority of professionals to work from home, disconnecting developers and managers from their usual workplaces and teams. Unfortunately, work-related anxiety and mental disorders are common among tech employees, and deteriorating mental health threatens the well-being of employees and the companies’ overall productivity. 
%Retaining developers in today’s ``Great Resignation'' era requires companies to build a team culture that allows for workforce engagement without inducing high stress and burnout. Work satisfaction is key factor to avoid attrition, representing a known predictor of employees' intentions to stay with their employer. However, it is still unknown the role that culture plays in the satisfaction of software delivery teams. 
%This study presents an empirical study of software delivery teams by analyzing the association between a variety of factors (Climate for Learning, Organizational Culture, Sense of Belonging, and Inclusiveness) to Work Satisfaction and Reduced Burnout. We test a theoretical model to shed light on how these factors relate using a survey with members of software delivery teams (n=3,281) working at Globant, a large multi-national company. 


%Burnout can be primarily reduced by focusing on team satisfaction for women, and satisfaction with Globant for men.
%, and find support for our hypotheses. In order to assess the moderating effects of roles, we adopt a multi-group approach using two groups of managers and team members. 

FROM INTRODUCTION
% Evidence suggests focusing on burnout prevention to achieve higher levels of employee functioning, justifying widespread research interest in identifying and managing their antecedents \cite{albrecht2015challenge,sabagh2018antecedents,roskam2020gender}.
% Many companies make considerable investments in employees’ well-being. 
%People generally spend most of their active time in a workplace, and a good workplace is clearly desirable. 
%and workplaces influence several factors at an individual, community, and society level. 
%Protective working conditions contribute to employee motivation and performance. 

%Previous research showed that organizational culture influences work satisfaction, but claimed for more investigation about opening the box and showing the indirect contribution that organizational culture has in work satisfaction \cite{janicijevic2018influence}.

% Globant is a digital transformation company with a global presence in five continents, 17 countries, and 36 cities. 
% %Instead of fighting the differences, 
% Globant benefits from cultural similarities and continuously trains the talent pool on technical and social skills, and has several initiatives in place to retain talents and avoid attrition. The well-being of their employees is essential to Globant, and research on the factors associated with reduced burnout is part of the company's strategy to employ actions to proactively target those factors, and avoid burnout and attrition.

%Work satisfaction and well-being are interconnected concepts. 
%Work satisfaction represents how fulfilled developers feel with their work, whereas well-being refers to how happy they are, and how their work impacts their work satisfaction \cite{forsgren2021space}.

%There is a virtuous circle when it comes to the benefits of work satisfaction \cite{dora}. Besides being considered as part of productivity \cite{forsgren2021space}, work satisfaction can also be seen as a predictor for key outcomes of organizations, such as organizational performance and their ability to deliver software successfully \cite{forsgren2018accelerate,dora}. 
%Work satisfaction of software developers has received considerable attention in recent years \cite{francca2018motivation,sharma2020exploring,stol2022gamification}.
%Employees’ well-being is a social issue as well. More than 300 million people suffer from depression globally (WHO, 2018) and all opportunities possibly improving wellbeing at a societal level should be exploited (Eurostat 2015).

%DevOps presents a strategic advantage for organizations when compared with traditional software development methods (often called phase-gate or waterfall). For organizations hoping to capture market share and deliver value faster (or even just deliver software more safely and securely), DevOps promises both speed and stability, by combining activities of software development and delivery to enhance the speed of getting new software features to customers. This leads to higher customer satisfaction and profitability, which are important outcomes at the organization level. 

%However, executing a successful DevOps transformation is not always easy. Organizations and software products vary in maturity and implementation, making transformation efforts difficult to design and deploy across teams and organizations. For DevOps to truly deliver value, it must include more than just technologies and automation, but also process and culture.


%% relevant to the topic of burnout - not a whole lot, and some are shite, but still useful to cite here.
% \cite{Sonnentag1994}
% \cite{maudgalya2006workplace}
% \cite{moore2000one}
% \cite{Singh2011}
% \cite{mellblom2019connection}
% \cite{shropshire2012m}

%% I'm collecting relevant sources to build the story - ks.

%Previous research showed that organizational culture influences work satisfaction, but claimed for more investigation about opening the box and showing the indirect contribution that organizational culture has in work satisfaction \cite{janicijevic2018influence}. Moreover, previous research also has argued the need for exploring the relationship between satisfaction, and burnout \cite{tripp2016job}. In this paper, we contribute to this scientific body of knowledge by building a theoretical model to represent how the organizational culture exerts an indirect effect on satisfaction and burnout through a climate for learning, a sense of belonging, and inclusiveness. Therefore, we address the following research question:\\[.1in]
%\noindent \textit{\textbf{RQ1.} How do organizational culture and work satisfaction reduce burnout in software delivery teams?}\\

%
%We do not suggest that the concepts we use cannot also be applied to other companies, and indeed it is possible that the model might prove more broadly applicable. In this paper, we contribute to the scientific body of knowledge by providing a theoretical model of antecedents and consequences of work satisfaction in software delivery teams.
%
%\begin{itemize}
%    \item We develop a theoretical model of sense of virtual community in OSS and assess it through a survey.
%    \item We examine the moderating effects of power distance and financial compensation between each of the intrinsic motivations and the sense of virtual community.
%    \item We present the results of an confirmatory factor analysis of a construct to measure sense of virtual community in OSS
%\end{itemize}
%
%\section{DevOps}
%
% A traditional software company releases software products infrequently, and each release can include hundreds of new features and improvements. Because releases are infrequent, users can grow impatient waiting for each new release and are thankful when it finally arrives. Disappointment sets in, however, when bugs are found and features don’t work as expected. Under great stress and with great turmoil, an emergency release is produced and put into production (hurried through the regular release process, often achieved by skipping tests), which has still more bugs, and the process repeats with more emergency releases, leading to more frustration, stress, and disappointment. Worse yet, new business opportunities are missed or ignored because of doubt, uncertainty, and distrust in the IT department’s ability to deliver value \cite{wiedemann2019devops}.
%
%Such practices are a thing of the past for companies that subscribe to the DevOps method of software development and delivery. DevOps organizational approach stresses empathy and encourages greater collaboration between engineering teams involved in the software delivery, in order to provide better end user experience, reduce development time, enhance deployment frequency, increase stability, reduce change failure rate and optimize incident resolution time \cite{wiedemann2019devops}.
%
%The integration of Developer (Dev) and Operations teams (Ops) that work collaboratively to eliminate information silos \cite{makinen2016improving} represents the acronym DevOps. Following the agile principles of collaborative work (rather than a sequence of individual jobs) and of iterative development in short sprints, DevOps extends these principles to a broader perimeter than agile \cite{debois2008agile,forsgren2018accelerate}. A standard definition for DevOps is proposed in the IEEE Standard 2675-2021 \cite{ieee2021ieee} with a set of principles and practices that promote cooperation among key stakeholders to define, create, operate, and continuously improve systems, software or services. DevOps brings the culture of human collaboration across departments and automation \cite{leite2019survey} to facilitate making early changes to achieve higher delivery, quality and cooperation \cite{debois2008agile}.
%
%While a traditional software company tend to have organizational silos and release software products infrequently \cite{wiedemann2019devops}. the DevOps culture represents a shift toward collaboration between development, quality assurance, and operations \cite{tessem2008cooperation}. The goal of breaking those silos is to reduce the time that a change made to a system takes to be available to end users, while ensuring high quality and the least friction and blame between teams as opposed to trust and empathy \cite{riungu2016devops}. 
%
%A DevOps Capability is a part of skill and knowledge of an individual or team that gives the ability to execute a DevOps practice. A DevOps Practice is the act of carrying out a DevOps activity, or a portion of a process \cite{amaro2022capabilities}. DevOps Capabilities are categorized into Cultural, Technical, Measurement, and Process, and can be determined by the knowledge and combined skills of the team members \cite{dora}. While the team acquires skills related to the DevOps Capabilities, they are able to execute the Practices and result in DevOps Outcomes and results \cite{rodriguez2019advances}. The combination of Practices and Capabilities that lead to Outcomes are very extensive. In the present study, we focus on the following concepts from DORA Research Program \cite{dora}: Organizational Culture, Satisfaction, and Software Delivery Stability.
%
%\section{Background and Related Work}
%
%Culture represents a complex topic, hard to be formalized, hence the need to propose tools for measuring, evaluating, and predicting cultural behavior of thinking and acting \cite{furnham2012psychology}. 
%





%\textsc{Perceived Burnout:} 
%The term “burnout” was created to describe a condition experienced by people in the helping professions that is characterized by overwork resulting in exhaustion and fatigue \cite{freudenberger1974staff}. Burnout often manifests itself as a feeling of helplessness, and is correlated with pathological cultures and unproductive, wasteful work. This feeling can make the things we once loved about our work and life seem insignificant and dull. The Maslach Burnout Inventory (MBI) refers to three dimensions of burnout that include exhaustion, cynicism, and inefficacy \cite{maslach1997maslach}. Some organizational risk factors can predict burnout: being overloaded by work, not being able to influence decisions that affect own work, insufficient rewards, working at an unsupportive environment, perceiving an absence of fairness in decision-making processes and mismatching between organizational values and the individual’s values \cite{maslach2008early}.



%\subsection{Software Delivery Performance} 

%DORA Research Program \cite{dora} uses two metrics to evaluate the software delivery performance in terms of stability (time to restore services and change failure rate) and two metrics for velocity (lead time for changes and deployment frequency). The time to restore is the amount of time the team takes from detecting a user-impacting incident to having it remediated. The change failure rate is the rate of errors in delivered software, and is measure of the quality of the release process. The lead time of code changes is about how long does it take to go from ``code committed" to ``code successfully running in production" and the deploy frequency is about how often does the team deploy code \cite{forsgren2018accelerate}. 



%Because releases are infrequent, users can grow impatient waiting for each new release and are thankful when it finally arrives. Disappointment sets in, however, when bugs are found and features don’t work as expected. Under great stress and with great turmoil, an emergency release is produced and put into production (hurried through the regular release process, often achieved by skipping tests), which has still more bugs, and the process repeats with more emergency releases, leading to more frustration, stress, and disappointment. Worse yet, new business opportunities are missed or ignored because of doubt, uncertainty, and distrust in the IT department’s ability to deliver value \cite{wiedemann2019devops}.

%DevOps is then a culture, movement or Practice emphasized on collaboration and communication, focused on improving the software release cycle speed to production and build automation of new software components, while keeping high quality, mentioned in Lwakatare et al. [17], where a literature review on the term DevOps concludes that DevOps is a change of mindset substantiated with a set of automated Practices to encourage cross-functional team collaboration.





==> macros.tex <==
\newcommand{\nb}[2]{
	{
		{\color{black}{
				\small\fbox{\bfseries\sffamily\scriptsize#1}
				{\sffamily\small$\triangleright~${\it\sffamily\small #2}$~\triangleleft$}
	}}}
}

\ifdraft
\newcommand\grex[1]{\nb{Gregorio}{\color{red}#1}}
\newcommand\anita[1]{\nb{Anita}{\color{blue}#1}}
\newcommand\igor[1]{\nb{Igor}{\color{purple}#1}}
\newcommand\christoph[1]{\nb{Christoph}{\color{olive}#1}}
\newcommand\marco[1]{\nb{\color{red}Marco}{\color{blue}#1}}
\newcommand\bianca[1]{\nb{Bianca}{\color{purple}#1}}
\newcommand\georg[1]{\nb{Georg}{\color{olive}#1}}

\newcommand{\fixme}[1]{{\textcolor{red}{[FIXME] #1}}\xspace}
\newcommand{\cn}{{\color{violet}[citation required]}}
\newcommand{\tbd}{{\color{red}[To Be Done!]}}

\else
\newcommand\grex[1]{}
\newcommand\igor[1]{}
\newcommand\christoph[1]{}
\newcommand\marco[1]{}
\newcommand\bianca[1]{}
\newcommand\anita[1]{}
\newcommand\georg[1]{}

\newcommand{\fixme}[1]{}
\newcommand{\cn}{}
\newcommand{\tbd}{}

\fi
\let\labelindent\relax

\newcommand\iteration[1]{\vspace{3mm}\noindent\textbf{#1}\vspace{3mm}}

\newcommand{\grey}{\rowcolor{Gray}\bfseries}
\newcommand\setrow[1]{\gdef\rowmac{#1}#1\ignorespaces}
\newcommand\clearrow{\global\let\rowmac\relax}
\clearrow



